A Variational EM Algorithm for the Separation of Time-Varying Convolutive Audio Mixtures

This paper addresses the problem of separating audio sources from time-varying convolutive mixtures. We propose a probabilistic framework based on the local complex-Gaussian model combined with non-negative matrix factorization. The time-varying mixing filters are modeled by a continuous temporal stochastic process. We present a variational expectation-maximization (VEM) algorithm that employs a Kalman smoother to estimate the time-varying mixing matrix, and that jointly estimate the source parameters. The sound sources are then separated by Wiener filters constructed with the estimators provided by the VEM algorithm. Extensive experiments on simulated data show that the proposed method outperforms a block-wise version of a state-of-the-art baseline method.

==> coverletter-R1.tex <==
\pagestyle{empty}
\onecolumn

\begin{coverletter}{A Variational EM Algorithm for the Separation\\ of Time-Varying Convolutive Audio Mixtures}{T-ASL-05455-2015}

\begin{answereditor}{Given the recommendations and comments of the reviewers I reccommend major revisions.}
Based on the reviewers comments we prepared a revised manuscript. The major revisions are the followings:
\begin{itemize}
 \item We incorporated a number of clarifications, as suggested by R1 and R2.
 \item We perform a novel set of \textbf{experiments with blind initialization} of both the proposed and baseline methods, namely realistic 
initializations based alone on information contained in 
the mixture.
 \item We compared the proposed and baseline methods using real recordings, including an in-depth description of the experimental protocol, data recordings, and performance scores.
 \item  Additionally, we simplified the introduction of matrix $\mathbf{U}_{f\ell}$ in Section~\ref{sec:ESstep}. We actually replaced the former $\mathbf{U}_{f\ell}^\top$ with the new $\mathbf{U}_{f\ell}$. This enables us to remove the transpose operator in all subsequent equations involving $\mathbf{U}_{f\ell}$, and thus slightly simplify these equations. 

 \end{itemize}
We believe that we carefully addressed all the concerns of the two reviewers, in particular the addition of experiments with real data, as suggested by R2. Please find below detailed answers to the reviewers questions and comments.

\textbf{An annotated version of the revised manuscript, in which the modifications, novel paragraphs and sections are highlighted in green and numbered C1, C2, etc., is attached at the end of this "replies to reviewers". The authors' replies refer to these annotations, e.g., C4 on P4, means that annotation C4 can be found on page 4}. 

\end{answereditor}

\begin{answerreviewer}[Recommendation: Author Should Prepare A Minor Revision]

\qa{This paper addresses the difficult problem of convolutive and underdetermined audio source separation, in the very challenging context of 
time-varying mixing filters. The proposed contribution is very original and interesting, and the experimental results are convincing. Besides, the 
paper is very clear and well written. I thus support its publication without reservation.}
{We are pleased to read these positive comments.}

\qa{Below I make a few comments and suggestions. The suggestions do not necessarily demand to modify the manuscript; 
I only expect a response letter from the authors. I let them decide if the manuscript deserves to be changed accordingly or not.}
{The modifications to the manuscript, if any, are marked-up and signaled in the detailed answers below.}

\qa{The proposed method relies on a variational approximation of the posterior probability distribution, where the filters are assumed independent from 
the sources. Have the authors tried a more radical approximation, such as the mean field approximation, where all scalar random variables are assumed 
independent? This approach would allow them to get rid of the computationally demanding Kalman smoother, leading to a lower complexity of the E-step. 
However the price for this complexity reduction is a less accurate approximation, which could require an increased number of iterations to reach the 
same performance. Therefore I am not sure whether the overall computational time would be reduced or not.}
{We agree that other variational approximations could be tested and, in general, there is no way to know a priori which one is better in terms of 
performance and overall complexity. The choice may highly depend on the application. In methods using variational approximation, the approximation 
(factorization of posterior densities) is generally limited to, basically, what is just necessary for further closed-form development, i.e. make the 
posterior densities tractable. Obviously this is to limit approximation errors. In the proposed method, assuming all random variables to be a 
posteriori independent would imply to assume also that the mixing matrices between two successive time frames are a posteriori independent. Yet we 
imposed them to be temporally dependent via \eqref{eq:temp2}. Thus, this seems somehow contradictory and, in our opinion, this 
justifies to keep the dependency of $\mathbf{A}_{f\ell}$ over the time frames and use the standard Kalman theory instead. In addition, even if one 
considers all scalar variables (i.e. $s_{j,f\ell}$ in $\mathbf{s}_{f\ell}$ and $A_{ij,f\ell}$ in $\mathbf{A}_{f\ell}, ~\forall j,i,f,\ell$) to be 
independent a posteriori, the computation of the parameters of the posterior distribution of $A_{ij,f\ell}$ still depends on the posterior 
distributions $q(A_{ij,f\ell-1})$ and $q(A_{ij,f\ell+1})$. This is due to the temporal model of the filters and we would like to highlight that this
is not in contradiction with the hypothesized statistical a posteriori independence. In conclusion, assuming statistical a posteriori independence of 
the mixing-filter matrix entries does not release us from the use of the Kalman forward-backward recursion, and therefore it is a risk of increasing the 
approximation error while keeping a similar complexity.
% 
% 
% , (the prior distribution of) the model still imposes dependencies between them.
% Let us see why, by calculating the approximating posterior distribution for $a_{ji,f\ell}$, i.e $q(a_{ij,f\ell})$.
% In mean-field, one has to only consider the prior-distributions on which $a_{ij,f\ell}$ appears, then apply Expectation to get rid of the other latent-variables
% that co-appear, and be left with a function of only $a_{ij,f\ell}$, which normalised gives $q(a_{ij,f\ell})$.
% We easily see that $a_{ij,f\ell}$ appears on three terms: $p(\mathbf{A}_{f\ell}|\mathbf{A}_{f\ell-1})$,
% $p(\mathbf{A}_{f\ell+1}|\mathbf{A}_{f\ell})$ and $p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})$.
% Clearly the transition terms depend respectively on $a_{ij,f\ell-1}$ and $a_{ij,f\ell+1}$.
% Thus in order to obtain $q(a_{ij,f\ell})$ one requires to know both (previous' iteration's) 
% posterior estimates of $q(a_{ij,f\ell-1}),q(a_{ij,f\ell+1})$ so to marginalise out $a_{ij,f\ell-1},a_{ij,f\ell+1}$ from the transition terms. 
% Therefore one needs to know both $q(a_{ij,f\ell-1}),q(a_{ij,f\ell+1})$ in order to compute $q(a_{ij,f\ell})$.
% This is nothing else than a forward-backward recursion expressed as an alternation between variational posteriors ...
% %-----------------------------------------------------------------------
% By factorising the posterior distribution to the level of scalar random-variables, one expects to obtain a simpler algorithm.
% The fact is that the VEM of such factorisation is terifically difficult to derive, and even if it sounds paralogical at a first thought,
% it will still contain a recursive filter-smoother over the posterior distribution of the filters (E-A).
% Let us see why by analysing the resulting E-step: The factorisation up to scalar-level means to assume that all of the entries $s_{j,f\ell},A_{ij,f\ell}$ of 
% $\mathbf{s}_{j,f\ell},\mathbf{A}_{f\ell}$ are a posteriori independent, or more formally:
% \begin{align*}
% q(\mathcal{H}) \approx \prod \limits_{f,\ell,j=1}^{F,L,J} q(s_{j,f\ell}) \prod \limits_{i=1}^I q(A_{ij,f\ell}).
% \end{align*}
% Let us try to calculate the approximand of one of these scalar r.vs , e.g $q(s_{j,f\ell})$.
% In a mean field assumption, to calculate the posterior of an r.v, here $s_{j,f\ell}$,
% one has to only consider the factors of the (joint prior probability distribution of the) model 
% that contain $s_{j,f\ell}$: 
% The complete joint prior distribution in our case writes
% \begin{align*}
% p\left(\mathcal{H},\left\{ \mathbf{x}_{f\ell} \right\}_{f,\ell=1}^{F,L}\right) = 
% %
% \prod \limits_{f,\ell,j=1}^{F,L,J} p(s_{j,f\ell})
% %
% \prod \limits_{f=1}^F p(\mathbf{a}_{:,f1}) \prod \limits_{\ell=2}^L p(\mathbf{a}_{:,f\ell}|\mathbf{a}_{:,f\ell-1})
% %
% \prod \limits_{f,\ell=1}^{F,L} p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell}).
% \end{align*}
% It is easy to see that $s_{j,f\ell}$ appears in two terms, specifically $p(s_{j,f\ell})$, $p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})$.
% The mean field approximation for $q(s_{j,f\ell})$ gives
% \begin{align}
% q(s_{j,f\ell}) \propto p(s_{j,f\ell}) \exp \left( \mathbb{E}_{q(\mathcal{H} / s_{j,f\ell}) } [ \log p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})]\right) \propto \\
% %
% \mathcal{N}_c\Bigg( s_{j,f\ell} ; 0, \sum \limits_{k \in \mathcal{K}_j} w_{fk} h_{k\ell} \Bigg) \times \\
% %
% \exp \Bigg( 
% \frac{\mathbf{x}^\hermitian}{\var_f} \Big(\mathbb{E}_{q(A_{1:I1:J,f\ell})}[\mathbf{A}_{f\ell}] \mathbb{E}_{q(s_{r \neq j,f\ell})}[ \mathbf{s}_{f\ell}] \Big)
% +
% % 
% \Big(\mathbb{E}_{q(A_{1:I1:J,f\ell})}[\mathbf{A}_{f\ell}] \mathbb{E}_{q(s_{r \neq j,f\ell})}[ \mathbf{s}_{f\ell}]\Big)^\hermitian \frac{\mathbf{x}_{f\ell}}{\var_f} 
% - \\
% \frac{1}{\var_f}\mathbb{E}_{q(A_{1:I1:J,f\ell}) q(s_{r \neq j,f\ell})}[\mathbf{s}_{f\ell}^\hermitian \mathbf{A}_{f\ell}^\hermitian \mathbf{A}_{f\ell} \mathbf{s}_{f\ell}]
% \Bigg).
% \end{align}
% Calculating the $\exp()$ term is not so trivial, because one has to express $\log p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})$
% as a function of $s_{j,f\ell}$ only, which involves marginalsing (computing the Expectation over surrounding variables) 
% which here are the other sources and filters for that $f,\ell$ point: $\{s_{r,f\ell}\}_{r\neq j},\{A_{ij,f\ell}\}_{ij}$.
% (In the end the $\exp()$ term has to be written as tryonym of the form $\exp( \alpha^\ast s_{j,f\ell} + \alpha s_{j,f\ell}^\ast - \beta |s_{j,f\ell}|^2)$ 
% so that when multiplied by $p(s_{j,f\ell})$, will resutl in $q(s_{j,f\ell})$ being a univariate Complex-Gaussian.)
% %
% Deriving, posterior approximands for the entries of a filter, e.g. $q(A_{ij,f\ell})$ is even more complicated as there are three terms on which $A_{ij,f\ell}$ appears
% in the joint prior distribution of the model, namely the transition from $\mathbf{A}_{f\ell-1}$, the observation term $p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})$,
% and the transition to $\mathbf{A}_{f\ell+1}$. In summary the variational approximand of $q(A_{ij,f\ell})$ would have to be calculated through
% \begin{align*}
% q(A_{ij,f\ell}) \propto \exp \Bigg(
% \mathbb{E}_{q(\mathcal{H}/A_{ij,f\ell})}[\log p(\mathbf{A}_{f\ell}|\mathbf{A}_{f\ell-1})]
% + \nonumber \\
% \mathbb{E}_{q(\mathcal{H}/A_{ij,f\ell})}[\log p(\mathbf{x}_{f\ell}|\mathbf{A}_{f\ell},\mathbf{s}_{f\ell})]
% %
% + \\
% %
% \mathbb{E}_{q(\mathcal{H}/A_{ij,f\ell})}[\log p(\mathbf{A}_{f\ell+1}|\mathbf{A}_{f\ell})]
% \Bigg).
% \end{align*}
% The transition probability from $\mathbf{A}_{f\ell-1}$ when marginalised over $\{A_{ij,f\ell-1}\}_{i,j=1}^{I,J}$ will give an expression that contains 
% the mean/covariance of $q(\mathbf{A}_{f\ell-1})$ of the previous VEM-iteration, consequently the term having $\mathbf{A}_{f\ell+1}$
% will give also terms that depend on the mean/covariance of $q(\mathbf{A}_{f\ell+1})$ at the previous VEM-iteration.
% Therefore to calculate $q(\mathbf{A}_{f\ell})$ one requires $q(\mathbf{A}_{f\ell-1})$ and $q(\mathbf{A}_{f\ell+1})$, which is an alternation, or in other words
% a recursion, and in specific an algorithmically sound forward-backward pass, i.e a Kalman-smoother.
% Therefore it may not be the case of an extreme computational simplification emergin by the scalar mean field factorisation.
% To summarise a completely-factorised VEM does not show some obvious structural-limitation of separation performance, 
% i.e it still has a Kalman-smoother and the posterior of a source $s_{j,f\ell}$ practically depends
% on all other sources, henceforth it may provide an alternative VEM-algorithm that could be benchmarked over the proposed methodology.
}

\qa{The proposed approach is based on a rather crude approximation of convolution products in the time-frequency domain as can be seen in equation 
(4), which only holds if the impulse responses of the filters are shorter than the analysis windows of the STFT. Can the authors comment about the 
impact of this approximation on the source separation performance?}
{This is absolutely right. We take this opportunity given by Reviewer 1 to discuss this point in the present cover letter, since this is a problem that is both important, 
and, to our feeling, largely overlooked in the literature, at least in the audio source separation literature. Still to our feeling, 
this is because i) this approximation is at the very basis of the vast amount of frequency-domain source separation techniques that have been 
proposed for more that two decades now, since it enables to largely simplify the expression of the mixture and thus open the way for efficient 
subsequent processes, and ii) there is no simple solution to overcome the approximation error. Therefore, if one wants to develop a 
TF-domain processing for convolutive mixture with an easy-to-manipulate expression, he/she simply has to ``accept'' this approximation, 
and the resulting error. Everything happens like researchers in the field (including us) think that the benefit of using this approximation 
is much larger than the drawback. In practice the resulting modeling error is ``blindly propagated'' in the subsequent processing, 
but in the ASS literature it is quite rarely mentioned and even less accurately quantified as a source of possible errors in the final output signal. 
In response to Reviewer 2's question, we just admit that we disgracefully adopt this line. The main reason for it is that it is very difficult 
to accurately characterize/``separate'' the error coming from the MTF approximation, the error coming from initialization (in the new experiments, both source 
localization and binary masking perform less well with reverberation), and the error coming from the statistical models (of sources and filters). 
However, we present and comment results with two different mixing filter length. This was already the case in the simulations with controlled 
initialization: we compared the performance over mixtures \emph{I-512-3} and \emph{I-4096-3}, where the impulse responses in \emph{I-4096-3} are $8$ 
times longer than the STFT analysis window. Naturally there is some performance degradation. This is somehow the case again with the new simulations 
with blind initialization (see answer to Reviewer 2): Here we use two different reverberation times.
Note that a few approaches have tried to overcome the convolutive-to-multiplicative approximation problem with more accurate (but of course more 
complex) representations, e.g. a two-dimensional convolution in the STFT domain in: 
\begin{itemize}
\item Avargel, Y. \& Cohen, I. (2007). System identification in the short-time Fourier transform domain with crossband filtering. IEEE Transactions on Audio, Speech, and Language Processing, 15(4), 1305-1319.
\item Talmon, R., Cohen, I. \& Gannot, S. (2009). Relative transfer function identification using convolutive transfer function approximation. IEEE Transactions on Audio, Speech, and Language Processing, 17(4), 546-555.
\item Badeau, R. \& Plumbley, M. D. (2014). Multichannel high-resolution NMF for modeling convolutive mixtures of non-stationary signals in the time-frequency domain. IEEE/ACM Transactions on Audio, Speech, and Language Processing, 22(11), 1670-1680.
\end{itemize}
And of course, time-domain methods or hybrid time- and frequency-domain methods can be developed.}

\qa{In equations (33), (37), (40), the way the update is written does not explicitly enforce nonnegativity. Therefore when the value becomes very 
small, there might be the risk that numerical errors lead to a negative value. Have the authors ever observed this phenomenon?}
{Interestingly we never observed negative deflations with any of these equations. At a first glance they seem to allow 
negative values to be assigned to strictly non-negative parameters, but the estimated values are always positive.
Eq. (33) is a summation of expectations of a norm:
\begin{align*}
\var_f = \frac{1}{LI} \sum \limits_{\ell=1}^L \mathbb{E}_{q(\mathbf{s}_{f\ell})q(\mathbf{a}_{:,f\ell})}\left[ 
\parallel \mathbf{x}_{f\ell} - \mathbf{A}_{f\ell} \mathbf{s}_{f\ell} \parallel^2_2
\right] =  \nonumber \\
%
\frac{1}{LI} \sum \limits_{\ell=1}^L \bigg( \mathbf{x}_{f\ell}^\hermitian \mathbf{x}_{f\ell} - \mathbf{x}_{f\ell}^\hermitian
\hat{\mathbf{A}}_{f\ell}\hat{\mathbf{s}}_{f\ell}
%
 - \big( \hat{\mathbf{A}}_{f\ell} \hat{\mathbf{s}}_{f\ell} \big)^\hermitian \mathbf{x}_{f\ell} +
\text{tr}\big\{\mathbf{U}_{f\ell} \mathbf{Q}^{\eta s}_{f\ell} \big\} \bigg).
\end{align*}
Therefore, as long as $q(\mathbf{a}_{:,f\ell})$ and $q(\mathbf{s}_{f\ell})$
are valid distributions (e.g. they do not have degenerate covariances), $\var_f$ is ensured to be non-negative.
A similar reasoning applies to (37): As long as $\symmat{\Sigma}^{\xi a}_{f\ell}$ is a valid covariance,
the update for $\symmat{\Sigma}^a_f$ will lead to a positive definite hermitian matrix. 
Eq. (40) is difficult to verify, though no deflations appeared.
Summarising, as we explicitly describe in the paper now (see \refcm{matrix-reg}), we only add a regularization offset ($10^{-7}$ and $10^{-7} 
\mathbf{I}_{2IJ}$) to the update of $\var_f$ (33) and of $\symmat{\Sigma}^{\xi a}_{f\ell}$ (21) respectively.}

\qa{Regarding the updates of the NMF terms $w_{fk}$ and $h_{kl}$, the authors suggest that these updates can be iteratively applied until convergence 
within every M-step. On the one hand this is not necessary (a single update would still lead to an increase of the log-likelihood), and on the other 
hand, I think that this strategy increases the risk to stay trapped in a local optimum of the cost function. Indeed, once $w_{fk}$ or $h_{kl}$ has 
converged to zero, it is no longer possible to escape from this value. Have the authors tried to apply only one update per iteration and observed any 
difference?}
{This is what we actually did: In practice the NMF update rule was applied only once (for each $w_{fk}$ and $h_{k\ell}$) at each EM iteration. This 
was not clearly described, and it is now clarified (see \refcm{nmf-iterations}).}

\qa{The computational complexity of the proposed method seems very high. How does it compare with the baseline method?}
{The issue of computational complexity is briefly discussed in Section IV.7. However, there was no comparison with the baseline method. 
We added a comparison of the computation times, see \refcm{comp-block-wise}.}

\qa{The performance of the proposed and baseline methods is evaluated according to the SDR and SIR criteria. Why has the also very common SAR 
criterion not be included in this evaluation?}
{We include SAR scores in the new 
set of experiments, please see Table~\ref{tab:blindinit}.}

\qa{I am not sure that the notation for matrix transposition and conjugate transposition has been properly introduced.}
{The notations are now clarified, see \refcm{transpose}.}

\qa{In page 9 of the one-column draft, line indexed 48, probability distribution $q(H|H_0)$ is referred to as the  ‘posterior distribution’ of a 
subset of the latent variables. Actually, it is only an ‘approximation’ of the posterior distribution. This issue is just a question of language, but 
I think that the authors should make it clear.}
{We clarified this issue and the language abuse in \refcm{q-approx-1} and the footnote after \refcm{q-approx-2}.}

\qa{In page 10, line indexed 5, it is said that the factorization over frequency and over time ``arises naturally from the prior distributions''. I 
suggest to add ``and from the observation model (4)''.}
{Done in \refcm{factorization}.}

\qa{In page 12, line indexed 42, it is said ``Using (3), the expectation in (23) computes''. I suspect that this result is rather based on (4) 
instead of (3).}
{Yes. Corrected in \refcm{expectation-corr}.}

\typo{In page 7, line indexed 50, the notation for the dummy variable f in the sum is the same as that of the frequency index in $w_{fk}$}
{We are unable to find the aforementioned sum.}

\typo{In page 30, lines indexed 35-36, ‘by’ should be replaced by ‘with’}
{Done.}

\typo{Lastly, a few typos have been left in this manuscript and still need to be fixed}
{Done.}
\end{answerreviewer}

\begin{answerreviewer}[Recommendation: Author Should Prepare A Major Revision]
\qa{This paper generalizes the audio source separation method proposed in [12], which is based on multi-channel non-negative matrix factorization 
(NMF), in order to deal with situations where speakers and microphones are moving. The generalization consists in replacing the time-invariant mixing 
matrix assumed in [12] with a Markov-chain time-varying mixing matrix. The parameters and the posteriors of the latent variables constituting the 
proposed generalized model are estimated with a variational EM algorithm. The generalization is straightforward, i.e., researchers with knowledge of 
Bayesian statistics and audio signal processing can easily derive the proposed algorithm although the derivation is cumbersome.}
{
% We agree that adding a (hidden!) Markov chain to an existing model is not a conceptual break-through. However, up to our knowledge we propose the 
% first method modeling the filters of a convolutive mixing process as temporally-linked continuous latent variables. Moreover, the focus of the paper 
% is to present in details the combination of [12] with a hidden Markov chain modeling the temporal evolution of the filters. We propose a theoretically 
% sound model and present the fully detailed derivation of a variational EM. Importantly, the results reported in the experimental validation show, not 
% only that this technical contribution is relevant to the audio and speech processing community, but also that we successfully managed to resolve all 
% practical problems we have encountered, as described in the implementation section. We think that the complete research approach (a theoretical model, 
% its associated algorithm, its practical implementation and its extensive evaluation) should not be regarded as trivial. A clear indication of this is 
% that [12] appeared in 2010, and for the last 6 years, to our knowledge, no other researcher has submitted the present generalization to the case of 
% moving sources for publication.
% DIO: The above answer is vengeance,
% its sole result will be to negatively predespose the reviewer to read the rest of the revised-paper.
% At least I see no reason or purpose for the following 3 arguments:
% %
% 1.) The fact that for 6 years no researcher has submitted the present model for publication, could very well
% imply that many tried, but they dropped it because it was not performing well ...
% %
% 2. "We think that the complete research approach (a theoretical model, its associated algorithm, its practical implementation and its extensive evaluation) should not be regarded as trivial",
% What is this answer? Did the reviewer insulted our mathematical skills, and we draw our weapons?
% Well it is perfectly fine with me that he finds the model trivial, that means that we explained it so simply that it looked straightfowrard. that is the purpose of a paper in the first place, isn't it?
% Evenmore for its own level knowledge the derivation is simple? So what? That is a generalisation of its personal opinnion and we should respect it, 
% and also this perfect, because that is what made long-standing algorithms stay alive until today! What is the reason of dislike?
% %
% 3. "We agree that adding a (hidden!) Markov chain to an existing model is not a conceptual break-through."
% What is this sentence? Did the reviewer ask to convince him that a Markov-Chain is an innovation?
% No, First of all Milliards of papers employ Kalman-algortihms. There is absolutely no innovation in ours, and I like to agree with the reviewer
% (maybe the very existence of the filters is irrelevant for separation, i.e Duong/Vincent model).
% The only think the reviewer asked is experiments!!!!!!!! Everything else is personal opinnion which I respect.
% %
% \textbf{I would compactify the previous answer to:}
% %
The addition of a (hidden) Markov chain to an existing model may not, indeed, be seen as an original contribution. We note however that the problem of separating moving sound sources has not received a lot of attention and that there are only a handful of papers that properly deal with this problem. The proposed formulation is indeed a generalization of [12]. We disagree with the reviewer that this generalization is straightforward. Reference [12] was published in 2010. We thoroughly studied the audio processing literature and we could not find the generalization that we propose in this paper, or any other generalization. Even if the idea of adding a hidden Markov model to describe the temporal evolution of the filters may be seen as straightforward, the formal derivation of the variational approximation, the design of the associated EM procedure, the fine tuning of this procedure, its practical implementation, and the in-depth experimental analysis of its behavior are not so straightforward. We believe that all these elements contribute substantially to  understand the audio-source separation problem and to provide a sound methodology.
%However, to the best of our knowledge we propose the first method modeling the filters of a convolutive mixing process as temporally-linked continuous latent variables. The focus of the paper is thus to present in details the combination of [12] with a hidden Markov chain modeling the temporal evolution of the filters. We note that [12] appeared in 2010, and for the last 6 years, to our knowledge, no other researcher has submitted the present generalization to the case of moving sources. We propose a theoretically sound model and present the fully detailed derivation of a variational EM. The results reported in the experimental validation show, not only that this technical contribution is relevant to the audio and speech processing community, but also that we successfully managed to resolve all practical problems we have encountered, as described in the implementation section. We believe that the complete research approach (a theoretical model, its associated algorithm, its practical implementation and its extensive evaluation) is an ensemble that makes a substantial contribution to the audio processing scientific community.
}

\qa{Since the proposed method uses a time-varying signal mixture model, it is obvious that the method outperforms the method of [12] in the 
simulations described in the paper. I would like to see results of more realistic experiments that use real recordings and no prior information that 
is unavailable in practice. The descriptions of the motivation and the derivation are clear enough. The paper needs modifications only in the 
experimentation section.}
{We followed this recommendation and carried out a novel set of experiments with blind initialization as well as an experiment with real recordings (see Section~\ref{sec:blind}). These additions also answer questions 3, 4 and 5 of the reviewer.
We agree that the proposed method is expected to outperform 
the method of [12] since the latter was designed for time-invariant mixing filters. However, we did not compare our method directly with [12]. Instead, we compared our method with a block-wise extension of 
[12]. This block-wise extension is referred to as the baseline method, hence the confusion of the reviewer. We also note that the vast majority of existing audio-source separation methods with time-varying filters adopt a block-wise approach.
This is clearly mentioned in the Introduction (see \refcm{new-exp-intro}) and in the description of the baseline method (see Section\ref{sec:setup3}).}

[NB: for the sake of clarity, we inverted the order of the next three questions]\\

\qa{Show at least one method for blindly initializing NMF parameters and perform an experiment with a fully bind setup. This should not be deferred 
to future work.}
{We addressed this request carefully, and we reorganized Section V accordingly. The simulations with controlled initialization presented in the first 
version of the paper are now in the first subsection of Section V. We added a new experimental subsection with fully blind initialization (Section 
\ref{sec:blind}). Importantly, this subsection also includes simulations with additive noise (see Question 4) and experiments with real recordings 
(see Question 5). As described in Section~\ref{sec:init2}, for the initialization of both mixing filters and NMF parameters, we adapted a recently 
proposed state-of-the art blind source separation method based on source localization and binary masking (new references [49,53]). We 
believe that this method is a good representative of a family of recently proposed probabilistic methods based on mixture models of acoustic feature 
distribution parameterized by source position (we completed the text with the references for these methods). One strength of the method-of-choice is 
that it exploits localization features at all frequencies simultaneously, ensuring global robustness as well as immunity to the well-known 
cross-frequency source permutation problem of frequency-domain source separation methods. 
% Another good point is that this method does not require to 
% be initialized \textcolor{red}{[NB: this should be mentioned in the manuscript!!!!]}. 
This method provides state-of-the art results for such type of 
underdetermined mixture in the static case, and we also explain in Section~\ref{sec:init2} how we adapted it to our dynamic setup on a block-wise basis. In addition, the source separation performance obtained by this method (measured on the output of the binary masking) provides an 
additional baseline for the performance of the proposed complete scheme in the blind configuration (i.e. plugging the proposed VEM onto the blind 
initialization).}

\qa{Add experimental results using real recordings. For example, you may ask three persons, each holding a loudspeaker, to walk around in a room and 
make an audio recording with a two-channel microphone array.}
{We also addressed this request. We made real recordings in a medium-size room with two microphones, involving moving participants: they actually speak while they move around, we did not use loudspeakers. As mentioned above, these recordings were processed with the proposed method (and 
baseline method) with blind initialization, providing a realistic experiment that is very rarely present in the audio source separation 
literature. These experiments are described in Section~\ref{sec:blind}, the performance are reported in Table~\ref{tab:blindinit}, and discussed in the text.}

\qa{Perform simulation experiments to compare the proposed and previous methods when there is strong additive noise.}
{The new simulations of Section~\ref{sec:blind} were made without and with additive white Gaussian noise at relatively strong level (SNR between sum of speech sources and AWGN is set to 4dB). The performance are reported in Table~\ref{tab:blindinit} and the effect of the noise on source separation performance is commented in the text.}

\qa{ In the right column of page 38, you state "continuous circular movements were simulated by interpolating the BRIRs at the sample level." This 
simulation method needs justification.}
{The interpolation of ``static'' (B)RIRs to simulate dynamic settings (moving sources, moving microphones or a combination of both) is a standard approach in the sound 
processing literature. Most of the time, a basic linear interpolation between time-domain BRIR samples is used and is sufficient to provide 
high-quality simulation. In the simulations of Section V.A. we extended this principle with a compensation of the inter-channel delay before the 
interpolation and a ``decompensation'' of this delay after the interpolation, which is just a refinement. We also applied the interpolation at the 
sample level, i.e. we generated one BRIR for each signal sample to be filtered. This leads to generate a huge amount of filters and in the experiments 
of Section V.B we interpolated the BRIRs provided by the RIR simulator with a simplest, more usual, and less demanding scheme (in terms of computation and memory). We perfectly understand the concern of Reviewer 2 to see the BRIR interpolation scheme justified, and maybe described in more detail. However we think that given the length of the paper, and given that the interpolation schemes we used provides high-quality simulated signals, we choose to not address this point extensively in the manuscript.}
\end{answerreviewer}


\end{coverletter}

\twocolumn
\setcounter{page}{1}
